PRBoost: Prompt-Based Rule Discovery and Boosting for Interactive Weakly-Supervised Learning

Weakly-supervised learning (WSL) has shown promising results in addressing label scarcity on many NLP tasks, but manually designing a comprehensive, high-quality labeling rule set is tedious and difficult. We study interactive weakly-supervised learning -- the problem of iteratively and automatically discovering novel labeling rules from data to improve the WSL model. Our proposed model, named PRBoost, achieves this goal via iterative prompt-based rule discovery and model boosting. It uses boosting to identify large-error instances and then discovers candidate rules from them by prompting pre-trained LMs with rule templates. The candidate rules are judged by human experts, and the accepted rules are used to generate complementary weak labels and strengthen the current model. Experiments on four tasks show PRBoost outperforms state-of-the-art WSL baselines up to 7.1% and bridges the gaps with fully supervised models. Our Implementation is available at \url{https://github.com/rz-zhang/PRBoost}.

==> others.tex <==
\subsection{Rule boosting derivation}
\label{boost_derive}

\subsection{Experiment Progress}
\noindent \textbf{Use weak sources for initialization}\\



\noindent \textbf{Improve the rule coverage}\\
Before:
Given the limited labeled dataset $\mathcal{D}_l$, we use boosting to find the top-k large errors $\mathcal{X}_e = \{x_{e_i}\}_{i=1}^k$.\\
Issue: With model initialization on weak sources, the newly proposed rules based on $\mathcal{X}_e$ easily overlaps with the weak labeled data.\\
Take dataset AGNews for example, the coverage of external weak sources is $56.4\%$, and the coverage of our proposed rules is $58.2\%$, while the overlapping calculated by the matched instance is $49.6\%$, which means only $8.6\%$ new instances got matched by the newly proposed rules.\\
So we turned to propose rules based on the instances unmatched by other weak sources. Specifically, we still leverage boosting to identify the top-k large errors $\mathcal{X}_e$ from $\mathcal{D}_l$, but we do not directly use $\mathcal{X}_e$ to do rule proposal. Instead, we find similar instances of $\mathcal{X}_e$ from the unmatched instances $\mathcal{D}_u$. Then the rule proposal part is based on those unmatched instances. In this way, the proposed rules matches $21.4\%$ new instances compared to the weakly labeled data. And the overall result on AGNews is $88.1\%$. \\

\noindent \textbf{Self-training}
To further improve the performance, we also implement self-training after the main framework completed, which brings a little performance improvement ($88.1\%$->$88.4\%$).

If we alternate between rule proposal, weak supervised learning and self training (for example, after 3-round rule proposal and weak supervised learning, we insert one self training ), the final performance achieves $88.7\%$.\\

\noindent \textbf{Issue of boosting}\\
During the experiments of baselines, I found the boosting itself is not able to bring performance improvement, if the initialized model can achieve a strong performance (i.e., on AGNews, the accuracy after initialization is $86.6\%$). Specifically, the weighted error rate of the initialized model is quite low, which makes its coefficient $\alpha$ very high compared to the following weak classifiers. For example, $\alpha_0 =3.0$ of the initialized model v.s. $\alpha_1 = 0.1$ of the new weak classifier.\\

\noindent \textbf{Some other baselines}\\
TALLOR (ACL21') This framework works only for NER problem.\\
LogiRE(EMNLP21') This paper has not been released till now.\\


\noindent \textbf{Label consistency}\\
For TACRED dataset, we consider propagate the label from the large errors identified on the limited training set to its most similar instance unmatched by the weak sources. We test the label propagation for the top-5 errors in 20 learning round, where the label consistency achieves 0.89/1. (measurement)\\

\noindent \textbf{Weaker sources, better improvement}\\
IWS $85.2\%->88.0\%$\\


\noindent \textbf{Self-training on each weak classifier}\\
$88.4\% -> 88.9\%$
If we do self-training for the weak classifiers trained only on the limited clean data, we find there is not much improvement to ensemble the weak-classifiers. For example,  $83.7\% -> 85.3\% -> 85.5\%$, the performance are the accuracy of weak classifier, self-trained weak classifier, and ensemble classifier, respectively. 


%How to leverage uncertainty to enable interactive weakly-supervised learning for spatial network classification? \\
Given a spatial network $\mathcal{G}$, we aim to predict its property by learning an uncertainty-aware classifier $C(y\mid\mathcal{G})$ from a set of training data points: $\mathcal{D} = \{\mathcal{G}_i, y_i\}_{i=1}^N$ and a set of unlabeled data points $\mathcal{D}_u$. This is challenging because the labeled data could be extremely limited in the real-world scenario, and conventional active learning can hardly provide scalable annotation by querying labels one by one. We thus propose to leverage uncertainty under the boosting paradigm to enable interactive weakly supervised learning for spatial network classification.\\

\begin{figure}[!htb]
    \centering
    \includegraphics[scale=0.5]{boost.pdf}
    \caption{The Framework of uncertainty-based boosting.}
    \label{fig:my_label}
\end{figure}
The proposed framework iteratively incorporates an uncertainty-aware model to the boosted model as 
$C_m(y\mid\mathcal{G}_i)=C_{m-1}(y\mid\mathcal{G}_i)+\alpha_mp_m(y\mid\mathcal{G}_i)$, for $m=1,2,\ldots,M$, where $C_m$ is the boosted model at the $m$-th iteration, and $p_m(y\mid\mathcal{G}_i)$ is the newly incorporated model. Since each component $p_m$ is able to output uncertainty, we can obtain an aggregated uncertainty for the boosted model $C_m$, which guides the following instance selection and the interpretable representation generation. We define the uncertainty score as $s(\cdot)$. Each iteration consists of the following stages as Fig. 1 shows:
(1) find the set $\mathcal{A}$ of high-uncertainty instances under the guidance of the boosted uncertainty-aware model, either by the top-$K$ selection $\mathcal{A}=\operatorname{argmax}_{D^{\prime} \subset D_u,\left|D^{\prime}\right|=K} \sum_{\mathcal{G} \in D^{\prime}} s(C(y\mid\mathcal{G}))$
, or the uncertainty threshold-based selection 
$\mathcal{A} = \{\mathcal{G}:s(C(y\mid\mathcal{G})<\eta\})$, where $\eta$ is the uncertainty lower threshold; 
(2) generate rationales $\mathbf{r}=\phi(A)$ for the selected instances, these rationales provide interpretability to the highly uncertain instances and will be presented to humans in the next stage;
(3) task humans for providing uncertainty-based feedback $h(\mathbf{r}) = h(\phi(\mathcal{A}))$ to the presented rationals;
(4) obtain weak labeled data using the human-evaluated rationales $h(\mathbf{r})$;
(5) train a weak model $p_m(y\mid\mathcal{G})$ and incorporate it into the boosted model if its model uncertainty $s(p_m(y\mid\mathcal{G}))$ is low, otherwise continue the weak annotation part.\\
These components are tightly-coupled and the benefits of the integral framework is three-fold. First, by equipping the ensemble model with uncertainty, we make the traditional boosting framework also uncertainty-aware, then the model uncertainty can guide the instance selection for the rationale generation. Second, the rationale generation enables the annotation at the feature level, which further improves the human-machine collaboration efficiency compared to labeling individual samples. Third, we integrate weak supervision with the boosting framework, where the human-evaluated rationales extrapolate to unseen data points for the weak learners training.
We describe below the key components in details.\\
\textbf{Boosted uncertainty-aware model $C(y\mid\mathcal{G})$.}
We put the uncertainty-aware model to the boosting framework, in order to aggregate uncertainty from a series of weak learners and iteratively select instances for querying annotation at the feature level, which enables reducing uncertainty obtained from a single weak learner. Specifically, we update a set of weights $w_i$ for the training data $\mathcal{D}$, where $i = 1,2,\ldots,N$. By calculating the weighted error rate of the weak learner as $\epsilon_{m}=\sum_{y_{i} \neq r_{m}\left(x_{i}\right)} w_{i}^{(m)} / \sum_{i=1}^{N} w_{i}^{(m)}$ and the uncertainty-guided weight of the weak learner as $\alpha_m = \frac{1-s(p_m(y\mid\mathcal{G}_i))}{2}\ln(\frac{1-\epsilon_m}{\epsilon_m})$, we are able to aggregate the uncertainty for the boosted model $C(y\mid\mathcal{G})$, while minimizing the total uncertainty of $C(y\mid\mathcal{G})$. This boosted model equipped with uncertainty can provide guidance for the following rationale generation.
\\
\textbf{Rationale generation $\mathbf{r}=\phi(\mathcal{A})$.}
The interactive setting requires a human-friendly representation to enhance the quality of human feedback. Here we use a mapping $\phi(\cdot)$ to generate rationales for the selected instances with high uncertainty. For the spatial network, the rationale could be a substructure or some other interpretable summarization of the network. There are multiple options for the mapping $\phi(\cdot)$: (1) it uses clustering methods to present typical cases among $\mathcal{A}$ to humans, then humans come up with salient rationales accordingly; (2) it uses pattern mining techniques to automatically discover the rationales of $\mathcal{A}$, then humans only need to evaluate them. Note that both ways ask humans for uncertainty-based feedback, i.e., the human proposed-rationales or the humans' feedback to the machine-discovered rationales come with a confidence score to indicate the uncertainty of rationales judged by humans. By mapping the set $\mathcal{A}$ to typical instances or rationales, humans can directly annotate at the feature level to reduce the labeling workload.
\\
\textbf{Training weak models}
We use techniques from weak supervision (\cite{,craven1999constructing, mintz2009distant, hoffmann2011knowledge, takamatsu2012reducing}) to obtain the weak learners. With the human-evaluated rationales $h(\mathbf{r})$, we can create weak labels for the unlabeled instances $\mathcal{D}_u$. We train a weak model $p(y\mid\mathcal{G})$ on the weakly labeled data and the original training set $\mathcal{D}$. The following operation depends on the uncertainty of $p(y\mid\mathcal{G})$: (1) The model with low uncertainty will be regarded as trustworthy and its own predictions will be used for self-training.  
(2) If the model uncertainty is unsatisfactory, the interactive data labeling will continue to reduce the model uncertainty by providing more supervision from the human side. 
\\
\textbf{Evaluation:} We plan to utilize popular benchmarks for spatial network classification such as the Gowalla check-in dataset \cite{cho2011friendship} and the Yelp check-in dataset \footnote{https://www.yelp.com/dataset challenge}. To compare with baselines, we apply the same annotation budget (calculated by annotation hours) to the models and evaluate the prediction performance. We can also study that to achieve the same performance as the baselines, how many annotations can be reduced by our method.

==> table/ablation.tex <==
\begin{tabular}{|p{1.5cm}<{\centering}|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}}\hline
     &2&4&6&8&10\\\hline
     supervised^\star  & \multicolumn{5}{c}{89.0}\\
     COSINE & \multicolumn{5}{c}{86.72} \\
     w/o ensemble & \multicolumn{5}{c}{87.74} \\
     w/o self-training & 87.16& 87.52& 87.80& 88.05& 88.27\\
     w/o rule& 86.95& 87.18& 87.32& 87.44& 87.48\\
     \textsc{PRBoost} & 87.40&  87.75& 88.26& 88.67&88.94 \\\hline
\end{tabular}

==> table/kolon.tex <==
\begin{tabular}{ccccc}\hline
    Supervision Type&Methods & TACRED & DBpedia & AG News  \\\hline
    \multirow{1}*{Supervised}&BERT w. 100\% training data&66.9 (66.3/67.6) &99.4 & 94.4\\
    \multirow{1}*{Weakly Supervised}& SOTA WS methods & 39.7 (39.2/40.1)^\dagger & 91.1^\ddagger&  87.5^*\\
    \multirow{1}*{Interactive Weakly Sup.}
    &Ours &48.1 (42.7/55.1) & 92.2  &88.9\\\hline
\end{tabular}

==> table/main_res.tex <==
\begin{tabular}{cccccc}\hline
    Supervision Type&Methods & TACRED & DBpedia & IMDB & AG News  \\\hline
    \multirow{3}*{Supervised}&BERT w. 100\% training data&66.9 (66.3/67.6) &99.4 &94.5 & 94.4\\
    &BERT w. 10\% training data & & & &\\
    &BERT w. 5\% training data & & & &\\\hline
    \multirow{4}*{Weakly Supervised}&LOTClass \cite{meng2020text}& &91.1 &86.5 &86.4\\
    % &UDA \cite{xie2019unsupervised}& &98.6 &88.7 &86.9\\
    &Snorkel \cite{ratner2017snorkel}& & & 73.2& 62.9\\
    &COSINE \cite{yu2020fine}& & &90.5 &87.5\\\hline
    \multirow{3}*{Interactive Weakly Sup.}&Active Learning &&&&\\
    &IWS \cite{boecking2020interactive}& & &87.3 &85.2\\
    &Ours &48.1 (42.7/55.1) & 90.3 & &86.8\\\hline
\end{tabular}


==> table/perf_iter.tex <==
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}\hline
     Iteration& 1& 2& 3& 4& 5& 6& 7& 8& 9& 10  \\\hline
     TACRED&  34.78& 37.55& 40.11& 42.27& 43.96& 45.45& 46.53& 47.47& 47.92& 48.28\\\hline
     Rule Coverage&\\
     Rule Accuracy&\\\hline\hline
     AGNews& 86.70& 87.07& 87.40& 87.75& 88.01& 88.26& 88.48& 88.67& 88.82 &88.94\\\hline
     Rule Coverage& 56.4& 60.1&	63.9& 67.1&	69.8& 72.5&	74.7& 76.1&	77.2& 77.8\\
     Rule Accuracy&83.10& 83.62&	84.09& 84.42& 84.68& 84.80&	85.15& 85.42& 85.58& 85.51\\\hline
\end{tabular}

==> table/rule_stats.tex <==
\resizebox{\textwidth}{10mm}
{
\begin{tabular}{c|c|c|c}\hline
       Dataset  & \# Rules & Coverage & Accuracy   \\\hline
        DBpedia     & 167 & 64.5 & 82.4\\
        AG News & 103 & 58.2 & 81.9\\\hline
\end{tabular}
}
